Large-scale linear hypothesis testing for high-dimensional online M-estimation

With the growing prevalence of streaming data, renewable estimation has become an important tool for updating statistical analyses without retaining historical raw observations. We study estimation and linear hypothesis testing in high-dimensional online M-estimation. Existing renewable procedures based on quadratic approximations can incur first-order approximation errors because the gradient of the unpenalized loss generally does not vanish at a preceding penalized estimator, posing a particular challenge for valid inference. To address this issue, we propose a corrected renewable loss that preserves historical first-order information and combine it with partial folded concave regularization and an iterative local linear approximation. We establish finite sample $\ell_1$- and $\ell_2$-error bounds, together with contraction bounds and strong oracle properties for both the constrained and unconstrained iterative estimators. Building on these results, we derive oracle Bahadur representations and establish asymptotically valid Wald and score tests for general linear hypotheses, allowing both the testing-oracle dimension and the number of restrictions to diverge. We further characterize their asymptotic power under local alternatives. The proposed procedure requires only recursively updated summaries while recovering the first-order inferential behavior of its pooled-data oracle counterpart. Simulation studies and real-data applications demonstrate the finite-sample performance of the proposed estimation and testing procedures.

==> preamble-shared.tex <==
\usepackage[margin=1in]{geometry}
\usepackage[dvipsnames]{xcolor}

\usepackage{amssymb, amsmath, amsthm, bm}
\usepackage{natbib}
\usepackage{microtype}
\setlength{\emergencystretch}{3em}
\usepackage{setspace}
\usepackage{rotating}
\usepackage{pdflscape}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{url}
\usepackage{enumitem}
\usepackage{pdfpages}
\usepackage{booktabs}
\usepackage{imakeidx}
\usepackage{authblk}

\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage{hypernat}

\usepackage{imakeidx}
\makeindex

\usepackage{booktabs}

\def\##1\#{\begin{align}#1\end{align}}
\def\$#1\${\begin{align*}#1\end{align*}}
\def\sn{\sum_{i=1}^n}

\makeatletter
\newcommand{\myitem}[1]{%
\item[#1]\protected@edef\@currentlabel{#1}%
}
\makeatother



%\bibliographystyle{minny}
\newcommand{\argmax}{\operatorname*{arg \ max}}
\newcommand{\argmin}{\operatorname*{arg \ min}}
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\DeclareMathOperator{\vol}{Vol}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\diam}{diam}
\global\long\def\inv#1{\frac{1}{#1}}
\DeclareMathOperator*{\Bias}{Bias}
\DeclareMathOperator*{\MSE}{MSE}
\DeclareMathOperator*{\Var}{Var}
\DeclareMathOperator*{\Cov}{Cov}
\DeclareMathOperator*{\Cor}{Cor}
\DeclareMathOperator*{\sd}{sd}
\def\T{{\sf \scriptscriptstyle{T}}}


%%%commands for remark and modification %%%
\newcommand{\remHDY}[1]{{\noindent (\color{WildStrawberry}#1 --Daeyoung)} \index{HDY}}
\newcommand{\modHDY}[1]{{\noindent  \color{OliveGreen}#1} \index{HDY}}

\newcommand{\remMY}[1]{{\noindent (\color{BrickRed}#1 --Myeonghun)} \index{MY}}
\newcommand{\modMY}[1]{{\noindent  \color{JungleGreen}#1} \index{MY}}

\newcommand{\remTAJ}[1]{{\noindent (\color{BlueViolet}#1 --Tate)} \index{TAJ}}
\newcommand{\modTAJ}[1]{{\noindent  \color{Purple}#1} \index{TAJ}}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\sub}{sub}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  Macros below here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\newcommand{\lp}{\left(} %% )
  \newcommand{\rp}{\right)}
\newcommand{\lb}{\left\{} %% )
  \newcommand{\rb}{\right\}}
\newcommand{\ls}{\left[} %% )
  \newcommand{\rs}{\right]}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}

\newcommand{\vp}{\varphi}


\newcommand{\ve}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\ve{#1}}

%% \newcommand{\cC}{\mathcal{C}} %% see below
\newcommand{\EE}{{\mathbb E}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\PPn}{{\mathbb P}_n}
\newcommand{\FFn}{{\mathbb F}_n}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\GGn}{{\mathbb G}_n}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{{\mathbb Z}}

\newcommand{\I}{\mathcal{I}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Gb}{\boldsymbol{\Gamma}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\scoreb}{\mathbf{s}}
\newcommand{\remb}{\mathbf{r}}
\newcommand{\Zb}{\mathbf{Z}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\Thetab}{\boldsymbol{\Theta}}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\omegab}{\boldsymbol{\omega}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\mub}{\boldsymbol{\mu}}



\newcommand{\eps}{\varepsilon}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\pp}{\ensuremath{\mathfrak{P}}}
\newcommand{\qq}{\ensuremath{\mathfrak{Q}}}
\newcommand{\mm}{\ensuremath{\mathfrak{M}}}
\newcommand{\ff}{\ensuremath{\mathcal {F}}}
\newcommand{\mbX}{\ensuremath{\mathbf {X}}}
\newcommand{\mbx}{\ensuremath{\mathbf {x}}}
\newcommand{\mbbeta}{\ensuremath{\pmb {\beta}}}
% \newcommand{\ff}{\ensuremath{\mathfrak{F}}}
\newcommand{\fft}{\ensuremath{\hat{\mathfrak{F}}}}
\newcommand{\ffn}{\ensuremath{{\mathfrak{F}}^{\otimes n}}}
\newcommand{\ffb}{\ensuremath{\ff_{\text{BDD}}}}
\newcommand{\ffs}{\ensuremath{\ff_{\text{SMU}}}}


\newcommand{\one}{\mathbbm{1}}
\newcommand{\mc}[1]{\mathcal {#1}}
\newcommand{\bb}[1]{\mathbb {#1}}
\newcommand{\kl}[2]{\rho_{\mathrm{KL}}\left({#1} \, \Vert \, {#2} \right)}

% \newcommand{\argmin}{\mathrm{argmin}}
%%\newcommand{\inf}{\mathrm{inf}}
%%\newcommand{\sup}{\mathrm{sup}}
\newcommand{\limsupp}{{\overline{\mathrm{lim}}}}
%% \newcommand{\width}{{\mathrm{width}}}
\newcommand{\SPAN}{{\mathrm{span}}}

\newcommand{\linaff}{\operatorname{Lin}}
%% \newcommand{\lin}{{\mathrm{lin}}}
\newcommand{\Lin}{\operatorname{Lin}}
\newcommand{\nn}{\nonumber}

\theoremstyle{plain}
\newtheorem{alg}{Algorithm}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem{corol}{Corollary}
\newtheorem{definition}{Definition}

\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}

\newtheorem{assumptionalt}{Assumption}[assumption]

% New environment
\newenvironment{assumptionp}[1]{
  \renewcommand\theassumptionalt{#1}
  \assumptionalt
}{\endassumptionalt}

\newcommand{\papertitle}{Large-scale linear hypothesis testing for
high-dimensional online M-estimation}

\providecommand{\blind}{0}


\newcommand{\paperkeywords}{Online inference; M-estimation; Linear hypothesis testing; Iteratively reweighted regression.}


% Anonymous rendering preserves editorial note text while omitting signatures.
\if0\blind
\renewcommand{\remHDY}[1]{{\noindent(\color{WildStrawberry}#1)}}
\renewcommand{\remMY}[1]{{\noindent(\color{BrickRed}#1)}}
\renewcommand{\remTAJ}[1]{{\noindent(\color{BlueViolet}#1)}}
\fi
\hypersetup{pdfauthor={},pdfsubject={},pdfkeywords={}}

\allowdisplaybreaks
